Mesh Draping: Parametrization-Free Neural Mesh Transfer

Despite recent advances in geometric modeling, 3D mesh modeling still involves a considerable amount of manual labor by experts. In this paper, we introduce Mesh Draping: a neural method for transferring existing mesh structure from one shape to another. The method drapes the source mesh over the target geometry and at the same time seeks to preserve the carefully designed characteristics of the source mesh. At its core, our method deforms the source mesh using progressive positional encoding. We show that by leveraging gradually increasing frequencies to guide the neural optimization, we are able to achieve stable and high quality mesh transfer. Our approach is simple and requires little user guidance, compared to contemporary surface mapping techniques which rely on parametrization or careful manual tuning. Most importantly, Mesh Draping is a parameterization-free method, and thus applicable to a variety of target shape representations, including point clouds, polygon soups, and non-manifold meshes. We demonstrate that the transferred meshing remains faithful to the source mesh design characteristics, and at the same time fits the target geometry well.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> figures/04_model_compare.tex <==

\newcommand\offsetx{1}
\newcommand\offsety{14}
\newcommand\starty{58.5}

\begin{figure}

\begin{overpic}[width=\columnwidth,tics=10, trim=0 0 190 0,clip]{figures/04_model_compare.png}

\put(\offsetx, 87.5){\Small{Source}}

\put(\offsetx,73){\Small{Target}}
% \put(\offsetx,77.5){\scriptsize{Chamfer ($\downarrow$)} }
% \put(\offsetx,76){\scriptsize{Dirichlet ($\downarrow$)}}

\put(\offsetx, \starty){\Small{Explicit}}
% \put(\offsetx,\fpeval{\starty -1.5}){\scriptsize{23.9}}
% \put(\offsetx,\fpeval{\starty - 3}){\scriptsize{14.03}}


\put(\offsetx, \fpeval{\starty - \offsety}){\Small{ReLU}}
% \put(\offsetx,\fpeval{\starty - \offsety -1.5}){\scriptsize{14.1}}
% \put(\offsetx,\fpeval{\starty - \offsety - 3}){\scriptsize{1.29}}

\put(\offsetx, \fpeval{\starty - 2 * \offsety}){\Small{Siren}}
% \put(\offsetx,\fpeval{\starty - 2 * \offsety -1.5}){\scriptsize{22.3}}
% \put(\offsetx,\fpeval{\starty - 2 * \offsety - 3}){\scriptsize{2.33}}


\put(\offsetx, \fpeval{\starty - 3 * \offsety}){\Small{PE}}
% \put(\offsetx,\fpeval{\starty - 3 * \offsety -1.5}){\scriptsize{16.6}}
% \put(\offsetx,\fpeval{\starty - 3 * \offsety - 3}){\scriptsize{1.55}}

\put(\offsetx, \fpeval{\starty - 4 * \offsety}){\Small{PPE}}
% \put(\offsetx,\fpeval{\starty - 4 * \offsety -1.5}){\scriptsize{6.65}}
% \put(\offsetx,\fpeval{\starty - 4 * \offsety - 3}){\scriptsize{1.7}}

\end{overpic}


     \caption{Mesh transfer comparison for different activation layers.}

     
     \label{fig:compare_model}
\end{figure}

==> tables/table_ppe_metrics.tex <==
\begin{table}
\centering%\footnotesize
% \vspace{-2pt}
% \ra{1.0}
\setlength{\tabcolsep}{2.99pt}
\begin{tabular}{@{}llcccccccccc@{}}
\toprule

\emph{Evaluation} && \multicolumn{2}{c} {\textbf{Alignment} ($1e^{-3})$} &  \textbf{Distortion} & \textbf{Joint} \\

  \emph{Metric} && Chamfer \scriptsize{($\downarrow$)} & Hausdorff \scriptsize{($\downarrow$)} & Dirichlet \scriptsize{($\downarrow$)} & \quality{} \scriptsize{($\uparrow$)} \\ \midrule
Explicit && 1.64 & 46.11 & 14.03 & 0.303 \\
  ReLU && 2.72 & 50.28 & \textbf{1.29} & 0.629  \\
  Siren && 14.10 & 79.79 & 2.33 & 0.461 \\
  PE && 3.17 & 55.15 & 1.55 & 0.594 \\
  PPE && \textbf{0.68} & \textbf{15.71} & 1.70 & \textbf{0.945}   \\
\bottomrule
\end{tabular}
\caption{
Quantitative ablation comparing our proposed PPE layer against other activation layers for the task of mesh transfer. Results are averaged over the shapes in Figure~\ref{fig:compare_model}.
\label{tab:activation_metrics}
}
% \vspace{-4mm}
\end{table}

